Non-Gaussianity constraints from Planck spectral distortion cross-correlations

Primordial non-Gaussianity can source $\mu$-distortion anisotropies that are correlated with the large-scale temperature and polarization signals of the cosmic microwave background (CMB). A measurement of $\mu T$ and $\mu E$ correlations can therefore be used to constrain it on wavelengths of perturbations not directly probed by the standard CMB anisotropies. In this work, we carry out a first rigorous search for $\mu$-type spectral distortion anisotropies with \Planck data, applying the well-tested constrained ILC component-separation method combined with the needlet framework. We reconstruct a $\mu$ map from \Planck data, which we then correlate with the CMB anisotropies to derive constraints on the amplitude $\fNL$ of the local form bispectrum, specifically on the highly squeezed configurations with effective wavenumbers $k_s \simeq \SI{740}{Mpc^{-1}}$ and $k_L \simeq \SI{0.05}{Mpc^{-1}}$. We improve previously estimated constraints by more than an order of magnitude. This enhancement is owing to the fact that for the first time we are able to use the full multipole information by carefully controlling biases and systematic effects in the final analysis. We also for the first time incorporate constraints from measurements of $\mu E$ correlations, which further tighten the limits. A combination of the derived \Planck $\mu T$ and $\mu E$ power spectra yields $|\fNL| \lesssim 6800$ (95\% c.l.) on this highly squeezed bispectrum. This is only $\simeq 3$ times weaker than the anticipated constraint from \LiteBIRD alone. We show that a combination of \LiteBIRD with \Planck will improve the expected future constraint by $\simeq 20\%$ over \LiteBIRD alone. These limits can be used to constrain multi-field inflation models and primordial black hole formation scenarios, thus providing a promising novel avenue forward in CMB cosmology.

==> tables/mock_cILC_forecast_LiteBIRD_FM.tex <==
\begin{tabular}{llll}
\toprule
$f_{\rm NL}$      &  Injected foregrounds     &   ILC Err. &  cILC (CMB removed) Err.\\
\midrule
25000 & CMB + Inst          & 319 & 319 \\
      & + Dust + Synch + FF & 909 & 909 \\
      & + tSZ + RS + IR     & 1207 & 1207 \\
12500 & CMB + Inst          & 252 & 252 \\
      & + Dust + Synch + FF & 898 & 898 \\
      & + tSZ + RS + IR     & 1197 & 1197 \\
0     & CMB + Inst          & 92 & 92 \\
      & + Dust + Synch + FF & 894 & 894 \\
      & + tSZ + RS + IR     & 1194 & 1194 \\
\bottomrule
\end{tabular}

==> tables/mock_cILC_forecast_Planck_FM.tex <==
\begin{tabular}{llll}
\toprule
$f_{\rm NL}$      &  Injected foregrounds     &   ILC Err. &  cILC (CMB removed) Err.\\
\midrule
25000 & CMB + Inst          & 1365 & 1365 \\
      & + Dust + Synch + FF & 2677 & 2677 \\
      & + tSZ + RS + IR     & 3009 & 3009 \\
12500 & CMB + Inst          & 1141 & 1141 \\
      & + Dust + Synch + FF & 2672 & 2672 \\
      & + tSZ + RS + IR     & 3005 & 3005 \\
0     & CMB + Inst          & 770 & 770 \\
      & + Dust + Synch + FF & 2670 & 2671 \\
      & + tSZ + RS + IR     & 3003 & 3003 \\
\bottomrule
\end{tabular}



==> tables/mock_cILC_forecast_Planck_HM.tex <==
\begin{tabular}{llll}
\toprule
$f_{\rm NL}$      &  Injected foregrounds     &   ILC Err. &  cILC (CMB removed) Err.\\
\midrule
25000 & CMB + Inst          & 1766 & 1766 \\
      & + Dust + Synch + FF & 3328 & 3328 \\
      & + tSZ + RS + IR     & 3660 & 3660 \\
12500 & CMB + Inst          & 1480 & 1480 \\
      & + Dust + Synch + FF & 3323 & 3324 \\
      & + tSZ + RS + IR     & 3656 & 3656 \\
0     & CMB + Inst          & 1089 & 1089 \\
      & + Dust + Synch + FF & 3322 & 3322 \\
      & + tSZ + RS + IR     & 3655 & 3655 \\
\bottomrule
\end{tabular}

==> tables/old/ideal_forecast_ilc_noise.tex <==
\begin{tabular}{lllll}
\toprule
$f_{\rm NL}$      &  Data                  &  Err. Ideal &  Err. est. frg. dgr. &  Err. real frg. \\
\midrule
25000 & $\mu$-T &        1365 &                 3097 &            3010 \\
      & $\mu$-E &        1073 &                 2705 &            2878 \\
      & $\mu$-T \& $\mu$-E &         957 &                 2343 &            2358 \\
12500 & $\mu$-T &        1141 &                 2684 &            3006 \\
      & $\mu$-E &         954 &                 2494 &            2873 \\
      & $\mu$-T \& $\mu$-E &         837 &                 2119 &            2354 \\
6250  & $\mu$-T &         967 &                 2450 &            3005 \\
      & $\mu$-E &         870 &                 2357 &            2871 \\
      & $\mu$-T \& $\mu$-E &         747 &                 1976 &            2353 \\
\bottomrule
\end{tabular}

